Privacy in Open Search: A Review of Challenges and Solutions

Privacy is of worldwide concern regarding activities and processes that include sensitive data. For this reason, many countries and territories have been recently approving regulations controlling the extent to which organizations may exploit data provided by people. Artificial intelligence areas, such as machine learning and natural language processing, have already successfully employed privacy-preserving mechanisms in order to safeguard data privacy in a vast number of applications. Information retrieval (IR) is likewise prone to privacy threats, such as attacks and unintended disclosures of documents and search history, which may cripple the security of users and be penalized by data protection laws. This work aims at highlighting and discussing open challenges for privacy in the recent literature of IR, focusing on tasks featuring user-generated text data. Our contribution is threefold: firstly, we present an overview of privacy threats to IR tasks; secondly, we discuss applicable privacy-preserving mechanisms which may be employed in solutions to restrain privacy hazards; finally, we bring insights on the tradeoffs between privacy preservation and utility performance for IR tasks.

==> bib.tex <==
\begin{thebibliography}{43}
\bibitem{wang2015collaborative}Wang, H., Wang, N. \& Yeung, D. Collaborative deep learning for recommender systems. {\em Proceedings Of The 21th ACM SIGKDD International Conference On Knowledge Discovery And Data Mining}. pp. 1235-1244 (2015)

\bibitem{sun2018data}Sun, W., Cai, Z., Li, Y., Liu, F., Fang, S. \& Wang, G. Data processing and text mining technologies on electronic medical records: a review. {\em Journal Of Healthcare Engineering}. \textbf{2018} (2018)

\bibitem{esposito2020hybrid}Esposito, M., Damiano, E., Minutolo, A., De Pietro, G. \& Fujita, H. Hybrid query expansion using lexical resources and word embeddings for sentence retrieval in question answering. {\em Information Sciences}. \textbf{514} pp. 88-105 (2020)

\bibitem{nguyen2018multilingual}Nguyen, H. \& Le Nguyen, M. Multilingual opinion mining on YouTube–A convolutional N-gram BiLSTM word embedding. {\em Information Processing & Management}. \textbf{54}, 451-462 (2018)

\bibitem{zhang2018tagvisor}Zhang, Y., Humbert, M., Rahman, T., Li, C., Pang, J. \& Backes, M. Tagvisor: A privacy advisor for sharing hashtags. {\em Proceedings Of The 2018 World Wide Web Conference}. pp. 287-296 (2018)

\bibitem{dai2020context}Dai, Z. \& Callan, J. Context-Aware Document Term Weighting for Ad-Hoc Search. {\em Proceedings Of The Web Conference 2020}. pp. 1897-1907 (2020)

\bibitem{pandey2018linear}Pandey, G., Ren, Z., Wang, S., Veijalainen, J. \& Rijke, M. Linear feature extraction for ranking. {\em Information Retrieval Journal}. \textbf{21}, 481-506 (2018)

\bibitem{zhuang2020counterfactual}Zhuang, S. \& Zuccon, G. Counterfactual Online Learning to Rank. {\em European Conference On Information Retrieval}. pp. 415-430 (2020)

\bibitem{zolaktaf2020facilitating}Zolaktaf, Z., Milani, M. \& Pottinger, R. Facilitating SQL Query Composition and Analysis. {\em Proceedings Of The 2020 ACM SIGMOD International Conference On Management Of Data}. pp. 209-224 (2020)

\bibitem{tao2020computing}Tao, Y., He, X., Machanavajjhala, A. \& Roy, S. Computing Local Sensitivities of Counting Queries with Joins. {\em Proceedings Of The 2020 ACM SIGMOD International Conference On Management Of Data}. pp. 479-494 (2020)

\bibitem{hadgu2020learn2link}Hadgu, A. \& Gundam, J. Learn2Link: Linking the Social and Academic Profiles of Researchers. {\em Proceedings Of The International AAAI Conference On Web And Social Media}. \textbf{14} pp. 240-249 (2020)

\bibitem{brickley2019google}Brickley, D., Burgess, M. \& Noy, N. Google Dataset Search: Building a search engine for datasets in an open Web ecosystem. {\em The World Wide Web Conference}. pp. 1365-1375 (2019)

\bibitem{magazine2017landscape}Magazine, D. The landscape of research data repositories in 2015: A re3data analysis. {\em D-Lib Magazine}. \textbf{23} (2017)

\bibitem{westin1968privacy}Westin, A. Privacy and freedom. {\em Washington And Lee Law Review}. \textbf{25}, 166 (1968)

\bibitem{EUdataregulations2018}Commission, E. 2018 reform of EU data protection rules. (\url{https://ec.europa.eu/commission/sites/beta-political/files/data-protection-factsheet-changes_en.pdf},2018), Date: 2018-05-25, URL Date: 2019-06-17

\bibitem{kaissis2020secure}Kaissis, G., Makowski, M., Rückert, D. \& Braren, R. Secure, privacy-preserving and federated machine learning in medical imaging. {\em Nature Machine Intelligence}. \textbf{2}, 305-311 (2020)

\bibitem{boulemtafes2020review}Boulemtafes, A., Derhab, A. \& Challal, Y. A review of privacy-preserving techniques for deep learning. {\em Neurocomputing}. \textbf{384} pp. 21-45 (2020)

\bibitem{zhang2020adversarial}Zhang, W., Sheng, Q., Alhazmi, A. \& Li, C. Adversarial attacks on deep-learning models in natural language processing: A survey. {\em ACM Transactions On Intelligent Systems And Technology (TIST)}. \textbf{11}, 1-41 (2020)

\bibitem{cash2015leakage}Cash, D., Grubbs, P., Perry, J. \& Ristenpart, T. Leakage-abuse attacks against searchable encryption. {\em Proceedings Of The 22nd ACM SIGSAC Conference On Computer And Communications Security}. pp. 668-679 (2015)

\bibitem{liu2020mitigating}Liu, H. \& Wang, B. Mitigating File-Injection Attacks with Natural Language Processing. {\em Proceedings Of The Sixth International Workshop On Security And Privacy Analytics}. pp. 3-13 (2020)

\bibitem{dai2019efficient}Dai, X., Dai, H., Yang, G., Yi, X. \& Huang, H. An efficient and dynamic semantic-aware multikeyword ranked search scheme over encrypted cloud data. {\em IEEE Access}. \textbf{7} pp. 142855-142865 (2019)

\bibitem{cramer_damgard_nielsen_2015}Cramer, R., Damgård, I. \& Nielsen, J. Secure Multiparty Computation and Secret Sharing. (Cambridge University Press,2015)

\bibitem{feng2020securenlp}Feng, Q., He, D., Liu, Z., Wang, H. \& Choo, K. SecureNLP: A System for Multi-Party Privacy-Preserving Natural Language Processing. {\em IEEE Transactions On Information Forensics And Security}. (2020)

\bibitem{dwork2008differential}Dwork, C. Differential privacy: A survey of results. {\em International Conference On Theory And Applications Of Models Of Computation}. pp. 1-19 (2008)

\bibitem{konevcny2016federated}Konečnỳ, J., McMahan, H., Yu, F., Richt\'arik, P., Suresh, A. \& Bacon, D. Federated learning: Strategies for improving communication efficiency. {\em NIPS Work- Shop On Private Multi-Party Machine Learning}. (2016)

\bibitem{carpineto2012survey}Carpineto, C. \& Romano, G. A survey of automatic query expansion in information retrieval. {\em Acm Computing Surveys (CSUR)}. \textbf{44}, 1-50 (2012)

\bibitem{nogueira2020document}Nogueira, R., Jiang, Z., Pradeep, R. \& Lin, J. Document Ranking with a Pretrained Sequence-to-Sequence Model. {\em Proceedings Of The 2020 Conference On Empirical Methods In Natural Language Processing: Findings}. pp. 708-718 (2020)

\bibitem{chuklin2015click}Chuklin, A., Markov, I. \& Rijke, M. Click models for web search. {\em Synthesis Lectures On Information Concepts, Retrieval, And Services}. \textbf{7}, 1-115 (2015)

\bibitem{act1996health}Act, A. Health insurance portability and accountability act of 1996. {\em Public Law}. \textbf{104} pp. 191 (1996)

\bibitem{gentry2009fully}Gentry, C. Fully homomorphic encryption using ideal lattices. {\em Proceedings Of The Forty-first Annual ACM Symposium On Theory Of Computing}. pp. 169-178 (2009)

\bibitem{chen2019federated}Chen, M., Suresh, A., Mathews, R., Wong, A., Allauzen, C., Beaufays, F. \& Riley, M. Federated Learning of N-Gram Language Models. {\em Proceedings Of The 23rd Conference On Computational Natural Language Learning (CoNLL)}. pp. 121-130 (2019)

\bibitem{qi-etal-2020-privacy}Qi, T., Wu, F., Wu, C., Huang, Y. \& Xie, X. Privacy-Preserving News Recommendation Model Learning. {\em Findings Of The Association For Computational Linguistics: EMNLP 2020}. pp. 1423-1432 (2020,11), https://www.aclweb.org/anthology/2020.findings-emnlp.128

\bibitem{mcmahan2017communication}McMahan, B., Moore, E., Ramage, D., Hampson, S. \& Arcas, B. Communication-efficient learning of deep networks from decentralized data. {\em Artificial Intelligence And Statistics}. pp. 1273-1282 (2017)

\bibitem{zhu2017differentially}Zhu, T., Li, G., Zhou, W. \& Philip, S. Differentially private data publishing and analysis: A survey. {\em IEEE Transactions On Knowledge And Data Engineering}. \textbf{29}, 1619-1638 (2017)

\bibitem{mivule2017data}Mivule, K. Data Swapping for Private Information Sharing of Web Search Logs. {\em Procedia Computer Science}. \textbf{114} pp. 149-158 (2017)

\bibitem{riazi2017prisearch}Riazi, M., Songhori, E. \& Koushanfar, F. PriSearch: Efficient search on private data. {\em 2017 54th ACM/EDAC/IEEE Design Automation Conference (DAC)}. pp. 1-6 (2017)

\bibitem{orso2017overlaying}Orso, V., Ruotsalo, T., Leino, J., Gamberini, L. \& Jacucci, G. Overlaying social information: The effects on users’ search and information-selection behavior. {\em Information Processing & Management}. \textbf{53}, 1269-1286 (2017)

\bibitem{zhou2008brief}Zhou, B., Pei, J. \& Luk, W. A brief survey on anonymization techniques for privacy preserving publishing of social network data. {\em ACM Sigkdd Explorations Newsletter}. \textbf{10}, 12-22 (2008)

\bibitem{weng2014privacy}Weng, L., Amsaleg, L., Morton, A. \& Marchand-Maillet, S. A privacy-preserving framework for large-scale content-based information retrieval. {\em IEEE Transactions On Information Forensics And Security}. \textbf{10}, 152-167 (2014)

\bibitem{tamine2018evaluation}Tamine, L. \& Daoud, M. Evaluation in contextual information retrieval: foundations and recent advances within the challenges of context dynamicity and data privacy. {\em ACM Computing Surveys (CSUR)}. \textbf{51}, 1-36 (2018)

\bibitem{el2021papir}El-Ansari, A., Beni-Hssane, A., Saadi, M. \& El Fissaoui, M. PAPIR: privacy-aware personalized information retrieval. {\em Journal Of Ambient Intelligence And Humanized Computing}. pp. 1-17 (2021)

\bibitem{yang2017differential}Yang, G. \& Zhang, S. Differential privacy for information retrieval. {\em Proceedings Of The ACM SIGIR International Conference On Theory Of Information Retrieval}. pp. 325-326 (2017)

\bibitem{devlin2019bert}Devlin, J., Chang, M., Lee, K. \& Toutanova, K. BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding. {\em Proceedings Of The 2019 Conference Of The North American Chapter Of The Association For Computational Linguistics: Human Language Technologies, Volume 1 (Long And Short Papers)}. pp. 4171-4186 (2019)

\end{thebibliography}
